CryptRISC: A Secure RISC-V Processor for High-Performance Cryptography with Power Side-Channel Protection

Cryptographic computations are fundamental to modern computing, ensuring data confidentiality and integrity. However, these operations are highly vulnerable to power side-channel attacks that exploit variations in power consumption to leak sensitive information. Masking is a widely used countermeasure, yet software-based techniques often introduce significant performance overhead and implementation complexity, while fixed-function hardware masking lacks flexibility across diverse cryptographic algorithms. In this paper, we present CryptRISC, the first RISC-V-based processor that combines cryptographic acceleration with hardware-level power side-channel resistance through an ISA-driven operand masking framework. Our design extends the CVA6 core with 64-bit RISC-V Scalar Cryptography Extensions and introduces two microarchitectural components: a Field Detection Layer, which identifies the dominant algebraic field of each cryptographic instruction, and a Masking Control Unit, which applies field-aware operand randomization at runtime. This enables dynamic selection of Boolean, affine, or arithmetic masking schemes based on instruction semantics, providing optimized protection across algorithms including AES, SHA-256, SHA-512, SM3, and SM4. Unlike prior approaches relying on static masking logic or software instrumentation, our method performs operand masking transparently within the execution pipeline without modifying instruction encoding. Experimental results show speedups up to 6.80$\times$ over baseline software implementations, with only a 1.86% hardware overhead relative to the baseline CVA6 core, confirming the efficiency and practicality of CryptRISC.

==> sections/Discussion.tex <==


% \textcolor{blue}{In this section, by addressing two key questions, we aim to delineate \fram's capabilities and evaluate the constraints of traditional side-channel countermeasures in cryptographic systems.}

% \textcolor{blue}{RQ1: What are the comparative impacts on system performance and security between \fram and traditional masking schemes?}

% \textcolor{blue}{Masked Logic involves dividing sensitive data into multiple independent shares to reduce power consumption data dependency, which often incurs significant area and performance overheads due to the additional circuitry required for managing these shares. In contrast, \fram strategically modifies the synthesis process to enhance PSC resistance without extensive circuit modifications, thereby minimizing the impact on area and performance. 
% To substantiate our claims, we first evaluate the area overhead of various first-order masking schemes for AES using the 45nm library. This comparison highlights the efficiency of different approaches in terms of silicon area utilization. The area is quantified in gate equivalences (GE), normalized to the area of a 2-input NAND gate, which serves as the base unit in the given standard cell library and typically defines the technology-dependent unit area in contemporary CMOS technologies. 
% Table \ref{table:compare} illustrates the comparison results and consists of three columns: the first column indicates the masking approach evaluated, and the second column specifies a measure of the silicon area consumed by each scheme in kilo gate equivalences (kGE). Lastly, the third column quantifies the extent of area enhancement \fram offers compared to the approach. The results are based on synthesized netlists for each scheme, revealing that \fram demonstrates the least area overhead and offers a significant improvement over other existing methods. This underscores the effectiveness of our proposed synthesis methodology in overcoming the major limitation posed by masking. }

% \begin{table}[h!]
% \caption{Comparison of implementation cost of existing masking schemes for AES.}
% \label{table:compare}
% \begin{tabular}{|c|c|c|}
% \hline
% Approach & \begin{tabular}[c]{@{}l@{}}Area in kGE\end{tabular} & \begin{tabular}[c]{@{}c@{}}Improvement\\ in Area\end{tabular}\\ \hline
% \fram & 4.51 &  - \\ \hline
% Changing of Guards \cite{askeland2022guarding} & 13.66 &  3.02 $\times$ \\ \hline
%  d + 1 Share Masking \cite{de2016masking} & 6.68 &  1.48 $\times$ \\ \hline
% Threshold Implementation \cite{bilgin2015trade} & 8.12 & 1.80 $\times$ \\ \hline
% 4-Share AES \cite{wegener2018first}& 7.60 &   1.68 $\times$\\ \hline
% 2-Share AES \cite{shahmirzadi2021re} & 7.71 &  1.70 $\times$ \\  \hline
% 3-Share AES \cite{sugawara20193} & 17.10 & 3.79 $\times$ \\ \hline
% \end{tabular}
% \end{table}

% \textcolor{blue}{Despite the intent of first-order masking to bolster security by diminishing data dependency, this method does not completely shield against PSC attacks. For a detailed evaluation, we consider an AES implementation that incorporates first-order masking, specifically utilizing a masked Sbox designed to obscure the relationship between the cryptographic key and observable power consumption \cite{shahmirzadi2021new}.
% It was observed that a typical DPA attack on this AES implementation exhibits a success rate of approximately 15\%. In the case of CPA, it achieves a success rate of around 18\%. 
% To provide a comparative perspective, we also evaluate \fram for the same AES implementation. Using \fram, PSC attack simulations reveal substantially lower success rates: approximately 5\% for DPA and 8\% for CPA. This marked improvement underscores \fram’s effectiveness in mitigating the vulnerabilities associated with first-order masking by integrating side-channel resistance at the synthesis level, offering a robust defense against both DPA and CPA. Thus, \fram demonstrates its potential as a more effective solution for cryptographic hardware designs, particularly in high-security environments where the demand for protection against PSC attacks is paramount.}


% \textcolor{blue}{
% RQ2: What is the impact of different side-channel countermeasures and \fram on the reliability and efficiency of cryptographic systems?
% }

% \textcolor{blue}{In the realm of side-channel countermeasures, while various techniques aim to secure cryptographic hardware, they often introduce considerable drawbacks.
% Dual-rail precharge logic is a technique that significantly increases the complexity of circuit design, as each bit of data is represented by two wires. This necessitates more complex logic and routing in the hardware, leading to increased area and power overhead due to the doubled circuitry \cite{morrison2014synthesis}. Ensuring a perfect balance in power consumption is challenging due to process variations and dynamic operational conditions. Random Voltage/Frequency Scaling aims to reduce side-channel leakage by varying the supply voltage or operating frequency unpredictably. While effective in adding noise to power measurements, this can lead to system transition time and energy overhead \cite{yang2012power}. Noise Injection involves adding random noise into the power supply or directly into the circuit to obscure leakage patterns \cite{das2017high}. This method can effectively increase the difficulty of mounting a successful side-channel attack but may also decrease circuit reliability and increase power consumption. \fram, in contrast, does not require additional power to inject noise as it modifies the synthesis of the netlist to inherently reduce leakages, offering a more reliability-friendly solution.}


==> sections/revision.tex <==
\begingroup
\color{blue}




\section{Discussion}
\label{sec:revision}

\subsection{Design Contributions and Architectural Novelty}

While CryptRISC builds upon the standardized RISC-V Scalar Cryptography Extensions, our contributions lie in its \textbf{field-aware operand randomization architecture}, which operates transparently at the microarchitectural level. We do not claim to invent new masking primitives; rather, we unify multiple masking styles---Boolean, arithmetic, and affine---into a single reconfigurable datapath driven by instruction semantics. This is accomplished through the integration of two components.

First, the \textbf{Field Detection Layer (FDL)} classifies each cryptographic instruction into its dominant algebraic domain using a lightweight lookup mechanism embedded in the decode stage.

Second, the \textbf{Masking Control Unit (MCU)} then uses this metadata to configure operand transformation dynamically, selecting the appropriate masking policy without modifying the ISA or the instruction encoding.

This architecture enables per-instruction operand masking without requiring software instrumentation or ISA-level annotations. In contrast to prior work that relies on software-inserted masking logic or fixed-function hardware masking, CryptRISC supports \emph{flexible field-specific countermeasures with runtime configurability}, making it both scalable and ISA-transparent.

\subsection{Relevance of Power Side-Channel Threats}

A recurring question is whether power side-channel attacks (PSCs) remain practical in the face of technology scaling. While it is true that shrinking process nodes decrease signal amplitude, they also concentrate switching activity into localized regions, which can increase signal-to-noise ratios under certain probes. Moreover, attackers increasingly use \textbf{EM probes} with sub-micron resolution, \textbf{statistical leakage analysis}, and \textbf{deep learning techniques} to amplify weak signals.

PSC attacks have been demonstrated in modern SoCs, particularly in \textbf{embedded platforms and IoT devices}, where physical access is common and masking remains one of the most effective first-order defenses. Our target threat model assumes such scenarios, where protection against physical side-channel leakage is mandatory.

\subsection{Updated Evaluation: Performance and Leakage Isolation}

In response to feedback on our evaluation methodology, we incorporated \textbf{two additional baselines}: (1) a baseline that includes \textbf{CVA6 with the RISC-V crypto ISEs but without masking}, to isolate the cost and benefit of masking logic alone; and (2) a comparison against \textbf{software-masked AES implementations}, which require manual instrumentation and offer limited extensibility.

Our results now demonstrate that CryptRISC achieves:
\begin{itemize}
    \item An average speedup of 4.76$\times$ over software-based crypto;
    \item Only 6--11\% performance overhead relative to unmasked ISE-accelerated execution, with no impact on critical path timing;
    \item Binary size reductions of up to 13.8\% by avoiding software masking expansions.
\end{itemize}

We also updated our side-channel evaluation with \textbf{instruction-level Test Vector Leakage Assessment (TVLA)} comparisons across three scenarios:
\begin{itemize}
    \item \textbf{Unmasked ISEs:} multiple instructions exceed the $\pm$4.5 leakage threshold;
    \item \textbf{Fixed-function masked cores (e.g., OpenTitan AES):} moderate suppression but vulnerable to higher-order attacks;
    \item \textbf{CryptRISC:} all evaluated instructions remain within $\pm$2 t-value range, indicating strong suppression of first-order leakage.
\end{itemize}

\subsection{Extensibility and Comparison to Alternatives}

A key advantage of CryptRISC is that its masking logic is \textbf{field-driven and decoupled from instruction formats}. Supporting new cryptographic algorithms, such as post-quantum primitives, simply requires extending the FDL’s lookup table with new field-tag mappings---no changes to datapath, control logic, or ISA are needed. This contrasts with fixed-function co-processors, which lack flexibility, or software masking, which incurs heavy programmer and compiler burden.

We also considered alternative defenses:
\begin{itemize}
    \item \textbf{Dummy operations and NOP injection}, which introduce performance overhead and do not generalize well to complex control/data dependencies;
    \item \textbf{Dual-rail encoding or threshold logic}, which require substantial circuit-level changes and are less portable across instruction sets;
    \item \textbf{Instruction scheduling techniques}, such as those proposed in PARADISE~\cite{paradise}, which reorder instructions to decorrelate leakage, but do not eliminate it. CryptRISC can be used \emph{in conjunction} with such schemes.
\end{itemize}

\subsection{Integration Transparency and Pipeline Analysis}

CryptRISC maintains a six-stage pipeline architecture (Fetch, Decode, Register Read, Execute, Memory, Write-Back). The \textbf{MCU is placed in the Execute stage}, immediately after operand fetch. As the operand randomization occurs within a single combinational cycle and does not depend on prior masked data, it does not affect the critical path. Synthesis at aggressive frequency targets confirms that maximum clock frequency remains unchanged compared to the baseline CVA6 core.

This transparent integration ensures that the CFU only receives \textbf{masked operands}, preventing data-dependent switching in sensitive logic. The pipeline remains fully compatible with existing compiler and toolchain support, offering secure execution with minimal software involvement.

\endgroup

==> sections/sss.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
% \usepackage{graphicx}
\begin{table}[]
\centering
\caption{}
\label{tab:my-table}
\resizebox{\columnwidth}{!}{%
\begin{tabular}{|c|ccc|lll|lll|}
\hline
\multicolumn{1}{|l|}{} &
  \multicolumn{3}{c|}{65 nm} &
  \multicolumn{3}{c|}{45 nm} &
  \multicolumn{3}{c|}{15 nm} \\ \hline
Benchmark &
  \multicolumn{2}{c|}{Success Rate} &
  \multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}Change \\ in Netlist\end{tabular}} &
  \multicolumn{2}{c|}{Success Rate} &
  \multicolumn{1}{c|}{\multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}Change \\ in Netlist\end{tabular}}} &
  \multicolumn{2}{c|}{Success Rate} &
  \multicolumn{1}{c|}{\multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}Change \\ in Netlist\end{tabular}}} \\ \cline{1-3} \cline{5-6} \cline{8-9}
 &
  \multicolumn{1}{c|}{\begin{tabular}[c]{@{}c@{}}Differential \\ Power \\ Analysis\end{tabular}} &
  \multicolumn{1}{c|}{\begin{tabular}[c]{@{}c@{}}Correlation \\ Power\\ Analysis\end{tabular}} &
   &
  \multicolumn{1}{c|}{\begin{tabular}[c]{@{}c@{}}Differential \\ Power \\ Analysis\end{tabular}} &
  \multicolumn{1}{c|}{\begin{tabular}[c]{@{}c@{}}Correlation \\ Power\\ Analysis\end{tabular}} &
  \multicolumn{1}{c|}{} &
  \multicolumn{1}{c|}{\begin{tabular}[c]{@{}c@{}}Differential \\ Power \\ Analysis\end{tabular}} &
  \multicolumn{1}{c|}{\begin{tabular}[c]{@{}c@{}}Correlation \\ Power\\ Analysis\end{tabular}} &
  \multicolumn{1}{c|}{} \\ \hline
AES\_Comp &
  \multicolumn{1}{c|}{0.05} &
  \multicolumn{1}{c|}{0.08} &
  19\% &
  \multicolumn{1}{l|}{1} &
  \multicolumn{1}{l|}{1} &
  1 &
  \multicolumn{1}{l|}{1} &
  \multicolumn{1}{l|}{1} &
  1 \\ \hline
AES\_TBL &
  \multicolumn{1}{c|}{0.10} &
  \multicolumn{1}{c|}{0.13} &
  15\% &
  \multicolumn{1}{l|}{1} &
  \multicolumn{1}{l|}{1} &
  1 &
  \multicolumn{1}{l|}{1} &
  \multicolumn{1}{l|}{1} &
  1 \\ \hline
AES\_PPRM1 &
  \multicolumn{1}{c|}{0.15} &
  \multicolumn{1}{c|}{0.20} &
  21\% &
  \multicolumn{1}{l|}{1} &
  \multicolumn{1}{l|}{1} &
  1 &
  \multicolumn{1}{l|}{1} &
  \multicolumn{1}{l|}{1} &
  1 \\ \hline
AES\_PPRM3 &
  \multicolumn{1}{c|}{0.12} &
  \multicolumn{1}{c|}{0.18} &
  20\% &
  \multicolumn{1}{l|}{1} &
  \multicolumn{1}{l|}{1} &
  1 &
  \multicolumn{1}{l|}{1} &
  \multicolumn{1}{l|}{1} &
  1 \\ \hline
RSA1024\_RAM &
  \multicolumn{1}{c|}{0.16} &
  \multicolumn{1}{c|}{0.21} &
  25\% &
  \multicolumn{1}{l|}{1} &
  \multicolumn{1}{l|}{1} &
  1 &
  \multicolumn{1}{l|}{1} &
  \multicolumn{1}{l|}{1} &
  1 \\ \hline
PRESENT &
  \multicolumn{1}{c|}{0.10} &
  \multicolumn{1}{c|}{0.15} &
  10\% &
  \multicolumn{1}{l|}{1} &
  \multicolumn{1}{l|}{1} &
  1 &
  \multicolumn{1}{l|}{1} &
  \multicolumn{1}{l|}{1} &
  1 \\ \hline
SABER &
  \multicolumn{1}{c|}{0.09} &
  \multicolumn{1}{c|}{0.12} &
  27\% &
  \multicolumn{1}{l|}{1} &
  \multicolumn{1}{l|}{1} &
  1 &
  \multicolumn{1}{l|}{1} &
  \multicolumn{1}{l|}{1} &
  1 \\ \hline
KYBER &
  \multicolumn{1}{c|}{0.14} &
  \multicolumn{1}{c|}{0.18} &
  22\% &
  \multicolumn{1}{l|}{1} &
  \multicolumn{1}{l|}{1} &
  1 &
  \multicolumn{1}{l|}{1} &
  \multicolumn{1}{l|}{1} &
  1 \\ \hline
\end{tabular}%
}
\end{table}
